Information-Guided Identification of Training Data Imprint in (Proprietary) Large Language Models

High-quality training data has proven crucial for developing performant large language models (LLMs). However, commercial LLM providers disclose few, if any, details about the data used for training. This lack of transparency creates multiple challenges: it limits external oversight and inspection of LLMs for issues such as copyright infringement, it undermines the agency of data authors, and it hinders scientific research on critical issues such as data contamination and data selection. How can we recover what training data is known to LLMs? In this work, we demonstrate a new method to identify training data known to proprietary LLMs like GPT-4 without requiring any access to model weights or token probabilities, by using information-guided probes. Our work builds on a key observation: text passages with high surprisal are good search material for memorization probes. By evaluating a model's ability to successfully reconstruct high-surprisal tokens in text, we can identify a surprising number of texts memorized by LLMs.

==> tables/all_dataset_contamination.tex <==
\begin{table*}[]

\begin{tabular}{lrrrrr} \\ \toprule
              & \multicolumn{1}{l}{Tokens} & CommonsenseQA & ARC & MMLU & Other Dataset \\ \midrule
Llama-2-70B & 100                        &    0.96\%         &             &                             &       \\
GPT-3.5 & 100                        &  6.73\%           &             &                             &      \\
GPT-4 & 100                        &   4.81\%          &             &                             &      \\
\bottomrule
\end{tabular}
\caption{}
\end{table*}

==> tables/all_dataset_contamination_filtered.tex <==
\begin{table}[]

\begin{tabular}{lrrrrr} \\ \toprule
              & \multicolumn{1}{l}{Tokens} & CommonsenseQA & ARC & MMLU_humanities \\ \midrule
Llama-2-70B & 100    &    0\%         &             &                                    \\
GPT-3.5 & 104  &  1.92\%           &             &                             &      \\
GPT-4 & 104   &   0.96\%          &             &                             &      \\
\bottomrule
\end{tabular}
\caption{}
\end{table}

%% Llama-3-70B           & 100                        & 2.88\%             &             &                             &       \\

==> tables/mmlu_contamination_c4_stats.tex <==

\begin{table}[tb]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll} \\ \toprule
MMLU subset & C4 contamination rate \\ \midrule
 abstract algebra  & 1.0\% (1/100)  \\
 anatomy  & 34.81\% (47/135)  \\
 business ethics  & 5.0\% (5/100)  \\
 clinical knowledge  & 3.02\% (8/265)  \\
 college chemistry  & 1.0\% (1/100)  \\
 college computer science  & 2.0\% (2/100)  \\
 college mathematics  & 6.0\% (6/100)  \\
 college medicine  & 5.78\% (10/173)  \\
 conceptual physics  & 4.68\% (11/235)  \\
 econometrics  & 0.88\% (1/114)  \\
 elementary mathematics  & 3.7\% (14/378)  \\
 formal logic  & 0.0\% (0/126)  \\
 global facts  & 3.0\% (3/100)  \\
 high school biology  & 4.84\% (15/310)  \\
 high school chemistry  & 14.78\% (30/203)  \\
 high school computer science  & 1.0\% (1/100)  \\
 high school european history  & 49.09\% (81/165)  \\
 high school geography  & 1.01\% (2/198)  \\
 high school government and politics  & 3.11\% (6/193)  \\
 high school mathematics  & 4.07\% (11/270)  \\
 high school microeconomics  & 8.4\% (20/238)  \\
 high school physics  & 13.91\% (21/151)  \\
 high school psychology  & 2.02\% (11/545)  \\
 high school statistics  & 6.48\% (14/216)  \\
 high school us history  & 72.06\% (147/204)  \\
 high school world history  & 50.21\% (119/237)  \\
 human aging  & 5.38\% (12/223)  \\
 human sexuality  & 1.53\% (2/131)  \\
 international law  & 6.61\% (8/121)  \\
 logical fallacies  & 3.07\% (5/163)  \\
 machine learning  & 5.36\% (6/112)  \\
 marketing  & 3.42\% (8/234)  \\
 medical genetics  & 7.0\% (7/100)  \\
 miscellaneous  & 4.21\% (33/783)  \\
 nutrition  & 0.0\% (0/306)  \\
 philosophy  & 0.96\% (3/311)  \\
 prehistory  & 0.93\% (3/324)  \\
 professional accounting  & 5.67\% (16/282)  \\
 professional medicine  & 0.74\% (2/272)  \\
 professional psychology  & 0.82\% (5/612)  \\
 public relations  & 1.82\% (2/110)  \\
 security studies  & 1.63\% (4/245)  \\
 virology  & 1.2\% (2/166)  \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/results_enron.tex <==
\begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength\tabcolsep{2.5pt}
\resizebox{.43\textwidth}{!}{
\begin{tabular}{lcccc}
\hline
\textbf{Identification Method} & \textbf{Precision} & \textbf{Recall} & \textbf{$F_{\beta}$} & \textbf{Document-level $F_{\beta}$} \\ \hline
random                                                             & 55.05                                      & \underline{49.57}                                & 7.88                                    & 15.32          \\ \hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-3.5} \\

verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
Surprisal (\emph{Person})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{BERT})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Llama-7B})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Mistal-7B-v0.1})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
\hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-4} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline

\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: Llama-2-70B} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline
% top-p (p=0.95) & \underline{95.63} & 56.16 & 18.58 & 63.73 \\ \hline %\cdashline{1-5}
% \ipam $\>$ (GPT-3) & 95.35 & \underline{57.26} & \underline{22.62} & \underline{71.40} \\
% \ipastar(GPT-3) & \textbf{96.26} & \textbf{61.94} & \textbf{32.84} & \textbf{73.17} \\ \hline
\end{tabular}
}
\caption{Identification results for GPT-3.5 (top), GPT-4 (centre), and LLama-2-70B (bottom) on \textit{fictional} text, with $\beta$=0.1.}
\label{tab:open-domain-auto}
% \vspace{-5mm}
\end{table}

==> tables/results_fiction_books.tex <==
\begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength\tabcolsep{2.5pt}
\resizebox{.43\textwidth}{!}{
\begin{tabular}{lcccc}
\hline
\textbf{Identification Method} & \textbf{Precision} & \textbf{Recall} & \textbf{$F_{\beta}$} & \textbf{Document-level $F_{\beta}$} \\ \hline
random                                                             & 55.05                                      & \underline{49.57}                                & 7.88                                    & 15.32          \\ \hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-3.5} \\

verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
Surprisal (\emph{Person})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{BERT})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Llama-7B})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Mistal-7B-v0.1})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
\hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-4} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline

\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: Llama-2-70B} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline
% top-p (p=0.95) & \underline{95.63} & 56.16 & 18.58 & 63.73 \\ \hline %\cdashline{1-5}
% \ipam $\>$ (GPT-3) & 95.35 & \underline{57.26} & \underline{22.62} & \underline{71.40} \\
% \ipastar(GPT-3) & \textbf{96.26} & \textbf{61.94} & \textbf{32.84} & \textbf{73.17} \\ \hline
\end{tabular}
}
\caption{Identification results for GPT-3.5 (top), GPT-4 (centre), and LLama-2-70B (bottom) on \textit{fictional} text, with $\beta$=0.1.}
\label{tab:open-domain-auto}
% \vspace{-5mm}
\end{table}

==> tables/results_fiction_sample_verticle.tex <==
                \begin{table}[t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.25}
\setlength\tabcolsep{2.5pt}
\resizebox{.43\textwidth}{!}{
\begin{tabular}{lcccc}
\hline
\textbf{Identification Method} & \textbf{Precision} & \textbf{Recall} & \textbf{$F_{\beta}$} &  \textbf{$F_{\beta}$ (Document)} \\ \hline
random                                                             & 50.17                                      & 50.51                               & 50.18                                   &           \\ 
majority                                                             & 49.84                                       & 100                                & 50.19                                    &          \\ \hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-3.5} \\

verbatim-tokensort  \newcite{duarte2024cop}                                                         & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs \newcite{karamolegkou2023copyright}                                                         & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP \newcite{duarte2024cop}                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
Surprisal (\emph{Person})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{BERT})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Llama-7B})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
Surprisal (\emph{Mistal-7B-v0.1})                                                               & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ 
\hline
\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: GPT-4} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline

\rowcolor[gray]{0.90} \multicolumn{5}{l}{\textit{Target Model}: Llama-2-70B} \\ 
verbatim-tokensort                                                           & 92.60                                      & 48.53                                      & 10.72                                   & 53.13          \\
verbatim-lcs                                                          & 95.85                                      & 47.61                                      & 13.24                                   & 56.42          \\
verbatim+replacement                                                        & 95.80                                      & 46.08                                      & 23.49                                   & \underline{63.92}    \\
verbatim+jailbreak                                                             & 95.67                                      & 46.12                                      & 23.67                                   & 62.21          \\
DE-COP                                                          & \underline{95.99}                                & 49.42                                      & \underline{36.73}                             & 61.95          \\ \hline % \cdashline{1-5}
\ipa (GPT2-XL)                                                                & \textbf{96.12}                             & \textbf{51.81}                             & \textbf{50.93}                          & \textbf{84.18} \\ \hline
% top-p (p=0.95) & \underline{95.63} & 56.16 & 18.58 & 63.73 \\ \hline %\cdashline{1-5}
% \ipam $\>$ (GPT-3) & 95.35 & \underline{57.26} & \underline{22.62} & \underline{71.40} \\
% \ipastar(GPT-3) & \textbf{96.26} & \textbf{61.94} & \textbf{32.84} & \textbf{73.17} \\ \hline
\end{tabular}
}
\caption{Identification results for GPT-3.5 (top), GPT-4 (centre), and LLama-2-70B (bottom) on \textit{fictional} text, with $\beta$=0.1.}
\label{tab:open-domain-auto}
% \vspace{-5mm}
\end{table}
